Deceptive Decision-Making Under Uncertainty

We study the design of autonomous agents that are capable of deceiving outside observers about their intentions while carrying out tasks in stochastic, complex environments. By modeling the agent's behavior as a Markov decision process, we consider a setting where the agent aims to reach one of multiple potential goals while deceiving outside observers about its true goal. We propose a novel approach to model observer predictions based on the principle of maximum entropy and to efficiently generate deceptive strategies via linear programming. The proposed approach enables the agent to exhibit a variety of tunable deceptive behaviors while ensuring the satisfaction of probabilistic constraints on the behavior. We evaluate the performance of the proposed approach via comparative user studies and present a case study on the streets of Manhattan, New York, using real travel time distributions.

==> preliminaries.tex <==
% \noindent\textbf{Notation:} The sets of 
% For a set $S$, we denote its cardinality by $\lvert S \rvert$. Additionally, $\mathbb{N}$$:=$$\{1,2,\ldots\}$, $\mathbb{R}$$:=$$(-\infty,\infty)$, and $\mathbb{R}_{\geq 0}$$:=$$[0,\infty)$. 
\section{Preliminaries}\label{prelim_sec}
 \noindent\textbf{Notation:} The sets of natural and real numbers are denoted by $\mathbb{N}$ and $\mathbb{R}$, respectively, while the set of nonnegative reals is denoted by $\mathbb{R}_{\geq 0}$. Finally, $|S|$ denotes the cardinality of a set $S$.
 %For a set $S$, we denote its cardinality by $\lvert S \rvert$. Additionally, $\mathbb{N}$$:=$$\{1,2,\ldots\}$, $\mathbb{R}$$:=$$(-\infty,\infty)$, and $\mathbb{R}_{\geq 0}$$:=$$[0,\infty)$. 

{\setlength{\parindent}{0cm}
\begin{definition}
A \textit{Markov decision process} (MDP) is a tuple $\mathcal{M}$$:=$$(S, s_1, \mathcal{A}, \mathcal{P})$ where $S$ is a finite set of states, $s_1$$\in$$S$ is an initial state, $\mathcal{A}$ is a finite set of actions, and $ \mathcal{P}$$:$$S$$\times$$ \mathcal{A}$$\times$$S$$\rightarrow$$[0,1]$ is a transition function such that $\sum_{s'\in S}\mathcal{P}(s,a,s')$$=$$1$ for all $s$$\in$$S$ and $a$$\in$$\mathcal{A}(s)$, where $\mathcal{A}(s)$$\subseteq$$\mathcal{A}$ denotes the set of available actions in $s$$\in$$S$.
\end{definition}}

We denote the transition probability $ \mathcal{P}(s,a,s')$ by $ \mathcal{P}_{s,a,s'}$. A state $s$$\in$$S$ is \textit{absorbing} if $\mathcal{P}_{s,a,s}$$=$$1$ for all $a$$\in$$\mathcal{A}(s)$. 
%The \textit{size of an MDP} is the number of triples $(s,a,s')$$\in$$S$$\times$$\mathcal{A}$$\times$$S$ such that $\mathcal{P}_{s,a,s'}$$>$$0$.

{\setlength{\parindent}{0cm}
\noindent \begin{definition}
\textcolor{red}{Switch to stationary, deterministic?} For an MDP $\mathcal{M}$, a \textit{policy} $\pi$$:=$$(d_1,d_2, d_3, \ldots)$ is a sequence where, for each $t$$\in$$\mathbb{N}$, $d_t$$:$$S$$\times$$\mathcal{A}$$\rightarrow$$[0,1]$ is a mapping such that $\sum_{a\in \mathcal{A}(s)}d_t(s,a)$$=$$1$ for all $s$$\in$$S$. A \textit{stationary} policy is a policy of the form $\pi$$=$$(d_1,d_1, d_1, \ldots)$. A stationary \textit{deterministic} policy is a stationary policy where, for each $s$$\in$$S$, $d_1(s,a)$$=$$1$ for some $a$$\in$$\mathcal{A}(s)$. We denote the set of all policies, all stationary policies, and all stationary deterministic policies by $\Pi(\mathcal{M})$, $\Pi^S(\mathcal{M})$, and $\Pi^{SD}(\mathcal{M})$, respectively. 
\end{definition}}

A policy $\pi$$\in$$\Pi(\mathcal{M})$ is traditionally referred to as a Markovian policy \cite{puterman2014markov}. Although it is possible to consider more general policy classes, the consideration of the set $\Pi(\mathcal{M})$ is without loss of generality for the purposes of this paper due to Theorem 5.5.1 in \cite{puterman2014markov}. For notational simplicity, we denote the probability of taking an action $a$$\in$$\mathcal{A}$ in a state $s$$\in$$S$ under a \textit{stationary} policy $\pi$ by $\pi(s,a)$.


A \textit{path} is a sequence $\varrho^{\pi}$$=$$s_1s_2s_3\ldots$ of states generated in $\mathcal{M}$ under $\pi$ which satisfies $\mathcal{P}_{s_t,a_t,s_{t+1}}$$>$$0$ for all $t$$\in$$\mathbb{N}$.
%, is called a \textit{path}. 
We define the set of all paths in $\mathcal{M}$ under $\pi$ by $Paths^{\pi}_{\mathcal{M}}$ and use the standard probability measure over the set $Paths^{\pi}_{\mathcal{M}}$ \cite{Model_checking}. Let $\varrho^{\pi}[t]$$:=$$s_t$ denote the state visited at the $t$-th step along the path $\varrho^{\pi}$, and $\bar{\rho}^\pi[t]\coloneqq s_1\dots s_t$. We define 
\begin{align*}
     \text{Pr}_{\mathcal{M}}^{\pi}(\mathsf{Reach}[B]):=\text{Pr}\{\varrho^{\pi}\in Paths^{\pi}_{\mathcal{M}}: \exists t\in \mathbb{N}, \varrho^{\pi}[t]\in B \}
\end{align*} 
as the probability with which the paths generated in $\mathcal{M}$ under $\pi$ reaches the set $B$$\subseteq$$S$.


